Parallel and Scalable Precise Clustering for Homologous Protein Discovery

This paper presents a new, parallel implementation of clustering and demonstrates its utility in greatly speeding up the process of identifying homologous proteins. Clustering is a technique to reduce the number of comparison needed to find similar pairs in a set of $n$ elements such as protein sequences. Precise clustering ensures that each pair of similar elements appears together in at least one cluster, so that similarities can be identified by all-to-all comparison in each cluster rather than on the full set. This paper introduces ClusterMerge, a new algorithm for precise clustering that uses transitive relationships among the elements to enable parallel and scalable implementations of this approach. We apply ClusterMerge to the important problem of finding similar amino acid sequences in a collection of proteins. ClusterMerge identifies 99.8% of similar pairs found by a full $O(n^2)$ comparison, with only half as many operations. More importantly, ClusterMerge is highly amenable to parallel and distributed computation. Our implementation achieves a speedup of 604$\times$ on 768 cores (1400$\times$ faster than a comparable single-threaded clustering implementation), a strong scaling efficiency of 90%, and a weak scaling efficiency of nearly 100%.

==> clustermerge.tex <==
\begin{figure}[]
    \centering
    \includegraphics[width=\columnwidth]{cluster_merge_fig}
    \caption{Cluster merge algorithm. Depending on the number of uncovered residues (U1, U2) and the alignment score, clusters
    are either fully merged (1-2), partially merged by exchanging matching sequences (3), or not merged at all.}
    \label{fig:clustermerge}
\end{figure}

==> cpu_util.tex <==

\begin{figure}[]
    \centering
    \includegraphics[width=0.9\columnwidth]{cpu_util_fig}
    \caption{CPU utilization with Shared-CM using 48 threads.}
    \label{fig:cpu_util}
\end{figure}
